RDF Translator: A RESTful Multi-Format Data Converter for the Semantic Web

The interdisciplinary nature of the Semantic Web and the many projects put forward by the community led to a large number of widely accepted serialization formats for RDF. Most of these RDF syntaxes have been developed out of a necessity to serve specific purposes better than existing ones, e.g. RDFa was proposed as an extension to HTML for embedding non-intrusive RDF statements in human-readable documents. Nonetheless, the RDF serialization formats are generally transducible among themselves given that they are commonly based on the RDF model. In this paper, we present (1) a RESTful Web service based on the HTTP protocol that translates between different serializations. In addition to its core functionality, our proposed solution provides (2) features to accommodate frequent needs of Semantic Web developers, namely a straightforward user interface with copy-to-clipboard functionality, syntax highlighting, persistent URI links for easy sharing, cool URI patterns, and content negotiation using respective HTTP headers. We demonstrate the benefit of our converter by presenting two use cases.

==> rdf-translator-3b-evaluation.tex <==
%% rdf-translator-3b-evaluation.tex

%	%================================================
%	\section{Evaluation}
%	\label{sec:evaluation}
%	%================================================
%	
%	\subsection{Validating the REST API}
%	
%	% HTTP GET for use with URIs, showing that content negotiation works
%	\begin{lstlisting}
%	$ curl -I http://rdf-translator.appspot.com/convert/detect/n3/http://www.stalsoft.com/grome
%	
%	HTTP/1.1 200 OK
%	Cache-Control: no-cache
%	Content-Type: text/n3
%	Access-Control-Allow-Origin: *
%	Content-Length: 0
%	Date: Mon, 24 Jun 2013 12:50:30 GMT
%	Server: Google Frontend
%	\end{lstlisting}
%	
%	(if a resource to convert does not exist, the service will throw a server error)
%	
%	(the service automatically follows 30x HTTP redirects)
%	
%	% HTTP POST for use with textual input and files
%	\begin{lstlisting}
%	$ curl --data-urlencode content="@prefix : <http://example.org/#> . :a :b :c ." http://rdf-translator.appspot.com/convert/n3/nt/content
%	\end{lstlisting}
%	
%	\begin{lstlisting}[caption={RDFa content}]
%	<div xmlns="http://www.w3.org/1999/xhtml"
%	  prefix="
%	    : http://example.org/#
%	    rdf: http://www.w3.org/1999/02/22-rdf-syntax-ns#
%	    rdfs: http://www.w3.org/2000/01/rdf-schema#"
%	  >
%	  <div typeof="rdfs:Resource" about="http://example.org/#a">
%	    <div rel=":b" resource="http://example.org/#c"></div>
%	  </div>
%	</div>
%	\end{lstlisting}
%	
%	\begin{lstlisting}
%	$ curl --data-urlencode content@example.rdfa http://rdf-translator.appspot.com/convert/rdfa/n3/content > example.n3
%	\end{lstlisting}
%	
%	\subsection{Validate the RDF Output}
%	
%	Compare systematically with the features of the other related tools presented in section 2!
%	
%	Features that come to my mind:
%	\begin{itemize}
%	\item Formats supported (input formats, output formats)
%	\item API? How to access it?
%	\item Usability: Syntax Highlighting? Persistent URI for sharing? Bookmarklets?
%	\item Verbosity (if something goes wrong, what errors are displayed, if any?)
%	\item Purpose (for testing, for production use, developed in accordance with standardization -> and therefore a prototype for testing, like for example Gregg Kellog's RDF Distiller)
%	\item Programming language (Python, Ruby, Java, ...)
%	\item RDF framework (RDFLib, ...) -> may witness for freshness, standards compliance
%	\item Kind of deployment: appspot, private server, ...
%	\item Other: e.g., incorporate data quality rules?
%	interestingly, Gregg Kellog has SPARQL support, but, to be honest, did not find out yet what the relation to the translation service is ...
%	\end{itemize}
%	
%	Compare output of the tools and validate! (http://www.delicious.com/kidehen/rdfizers)
%	
%	Validate using the following tools (Online):
%	\begin{itemize}
%	\item http://www.w3.org/TR/rdf-testcases/
%	\item http://swse.deri.org/RDFAlerts/ (http://pedantic-web.org/tools.html)
%	\item http://rdfa.info/test-suite/
%	\item http://foolip.org/microdatajs/live/
%	\item http://validator.nu/ or http://validator.w3.org/nu/ (http://www.w3.org/blog/SW/2012/02/08/new-w3c-validation-service-with-rdfa-1-1-and-microdata/)
%	\item http://validator.linkeddata.org/
%	\begin{itemize}
%	\item on http://rdf-translator.appspot.com/convert/rdfa/pretty-xml/http://www.stalsoft.com/
%	\item all tests passed!
%	\end{itemize}
%	\item http://www.w3.org/RDF/Validator/
%	\item http://www.rdfabout.com/demo/validator/
%	\item http://www.bing.com/toolbox/EntityExtraction
%	\end{itemize}
%	
%	Offline:
%	\begin{itemize}
%	\item http://librdf.org/raptor/rapper.html
%	\item http://incubator.apache.org/jena/documentation/io/riot.html
%	\item http://jena.sourceforge.net/Eyeball/
%	\item http://clarkparsia.com/pellet/
%	\end{itemize}
%	
%	Describe methodology, perhaps taking into account the features mentioned above... but argue why we selected these features for comparison and not others.

